Leveraging Hamilton-Jacobi PDEs with time-dependent Hamiltonians for continual scientific machine learning

We address two major challenges in scientific machine learning (SciML): interpretability and computational efficiency. We increase the interpretability of certain learning processes by establishing a new theoretical connection between optimization problems arising from SciML and a generalized Hopf formula, which represents the viscosity solution to a Hamilton-Jacobi partial differential equation (HJ PDE) with time-dependent Hamiltonian. Namely, we show that when we solve certain regularized learning problems with integral-type losses, we actually solve an optimal control problem and its associated HJ PDE with time-dependent Hamiltonian. This connection allows us to reinterpret incremental updates to learned models as the evolution of an associated HJ PDE and optimal control problem in time, where all of the previous information is intrinsically encoded in the solution to the HJ PDE. As a result, existing HJ PDE solvers and optimal control algorithms can be reused to design new efficient training approaches for SciML that naturally coincide with the continual learning framework, while avoiding catastrophic forgetting. As a first exploration of this connection, we consider the special case of linear regression and leverage our connection to develop a new Riccati-based methodology for solving these learning problems that is amenable to continual learning applications. We also provide some corresponding numerical examples that demonstrate the potential computational and memory advantages our Riccati-based approach can provide.

==> BC-versions/methodology.tex <==
\subsection{Regularized linear regression problems with quadratic integral-type losses}
\begin{figure}[htbp]

    \centering   
    \begin{adjustbox}{width=\textwidth}
\begin{tikzpicture}[node distance=2cm]
    \node (min) [nobox, yshift=-0.2cm] {$\min$};
    \node (minarg) [boxsmall, right of=min, xshift=-1.3cm, yshift=-0.42cm, draw=cyan!60, fill=cyan!5] {$\text{}_{\weightvec\in\weightspace}$};
    \node (sum) [nobox, right of=min, xshift=0.2cm] {$\mathlarger{\int}_0^t$};
    \node (loss) [box, right of=sum, xshift=0.1cm, draw=green!60, fill=green!5] {$\frac{\lambda}{2}\|\mathcal{A}\Phi(s)\weightvec - \MLy(s)\|_2^2$};
    \node(ds) [nobox, right of=loss, xshift=0.02cm] {$ds$};
    \node (plus) [nobox, right of=loss, xshift=0.5cm] {$+$};
    \node (regLeft) [nobox, right of=loss, xshift=4.35cm, draw=blue!60, fill=blue!5] {$\frac{\lambda_0}{2}\|\mathcal{B}_0\Phi(0)\weightvec - \bz_0\|_2^2 + \frac{\lambda_t}{2}\|\mathcal{B}_t\Phi(t)\weightvec - \bz_t\|_2^2$};
    \node (regularization) [nobox, right of=regLeft, xshift=1.8cm] {$+$};
    \node (regRight) [nobox, right of=regularization, xshift=0.0cm, draw=blue!60, fill=blue!5] {$\frac{1}{2}\sum_{i=1}^n\MLreg_i (\weight_i - \MLcenter_i)^2$};
    
    \node (sup) [nobox, below of=min, xshift=-0cm] {$\min$};
    \node (suparg) [boxsmall, right of=sup, xshift=-1.3cm, yshift=-0.44cm, draw=cyan!60, fill=cyan!5] {$\text{}_{\HJmom\in\HJstatespace}$};
    \node (sum2) [nobox, below of=sum,xshift=0cm]{$\mathlarger{\int}_0^t$};
    \node (equal) [nobox, left of=sup, xshift=1.4cm] {$=$};
    \node (S) [box, left of=equal, xshift=0.45cm, draw=red!60, fill=red!5] {$S(\MLregmat\MLcentervec, \HJt)$};
    \node (minus) [nobox, left of=S, xshift=0.9cm] {$-$};
    \node (Hamiltonian) [box, below of=loss, draw=green!60, fill=green!5] {$\frac{\lambda}{2}\|\mathcal{A}\Phi(s)\HJmom - \by(s)\|_2^2$};
    \node(HJds) [nobox, below of=ds, xshift=0cm] {$ds$};
    \node (plus2) [nobox, right of=Hamiltonian, xshift=0.75cm] {$+$};
    \node (IC) [box, below of=regLeft, draw=blue!60, fill=blue!5, xshift=-1.7cm] {$\frac{1}{2}\|M^{1/2}\HJmom\|_2^2$};
    \node (linear) [box, below of=regRight, draw=blue!60, fill=blue!5] {$-\langle \MLregmat\MLcentervec, \HJmom\rangle$};

    \node (OCmin) [nobox, below of=sup, xshift=0cm] {$\min$};
    \node (OCminarg) [boxsmall, below of=suparg, yshift=-0.01cm, draw=cyan!60, fill=cyan!5] {$\text{}_{\HJu(\cdot)}$};
    \node (OCS) [box, below of=S, xshift=0cm, draw=red!60, fill=red!5] {$S(\MLregmat\MLcentervec, \HJt)$};
    \node (leftbracket) [nobox, right of=OCmin, xshift=-0.65cm] {$\Bigg\{$};
    \node (OCequal) [nobox, below of=equal] {$=$};
    \node (OCint) [nobox, below of=sum2, xshift=-0.38cm] {$\mathlarger{\int}_0^t$};
    \node (OCHamiltonian) [box, below of=Hamiltonian, draw=green!60, fill=green!5] {$\frac{\lambda}{2}\HJu(s)^T\HJu(s) - \by(s)^T\HJu(s)$};
    \node (OCds) [nobox, right of=OCHamiltonian, xshift=0.415cm] {$ds$};
    \node (OCplus) [nobox, right of=OCds, xshift=-1.55cm] {$+$};
    \node (OCIC) [box, below of=IC, draw=blue!60, fill=blue!5] {$\frac{1}{2}\bx(t)^TM^{-1}\bx(t)$};
    \node (colon) [nobox, right of=OCIC, xshift=-0.53cm] {:};
    \node(OCdynamics) [box, right of=OCIC, xshift=2.25cm, draw=green!60, fill=green!5] {$\dot\bx(s) = (\mathcal{A}\Phi(s))^T\HJu(s), \forall s \in \left(0, \HJt\right]$};
    \node(comma) [nobox, right of=OCdynamics, xshift=0.6cm, yshift=-0.11cm] {,};
    \node (terminalposition) [box, right of=OCdynamics, xshift=1.95cm, draw=blue!60, fill=blue!5] {$\bx\left(0\right) = \MLregmat\MLcentervec$};
    \node (rightbracket) [nobox, right of=terminalposition, xshift=-0.72cm] {$\Bigg\}$};

    \node (LPequal) [nobox, above of=equal] {$=$};
    \node (minloss) [box, above of=S, draw=red!60, fill=red!5] {$\min_{\weightvec\in\weightspace}\mathcal{L}(\weightvec)$};
    
    \draw [doublearrow] (loss) -- (Hamiltonian);
    \draw [dottedarrow] (regLeft) -- (IC);
    \draw [dottedarrow] (regLeft) -- (linear);
    \draw [dottedarrow] (regRight) -- (IC);
    \draw [dottedarrow] (regRight) -- (linear);
    \draw [doublearrow] (minarg) -- (suparg);
    \draw [doublearrow] (S) -- (OCS);
    \draw [dottedarrow] (IC) -- (OCIC);
    \draw [dottedarrow] (Hamiltonian) -- (OCHamiltonian);
    \draw [dottedarrow] (Hamiltonian) -- (OCdynamics);
    \draw [dottedarrow] (linear) -- (terminalposition);
    \draw[dottedarrow](minloss) -- (S);
    \draw[dottedarrow] (suparg) -- (OCminarg);
\end{tikzpicture}
\end{adjustbox}

    \caption{(See Section~\ref{sec:method}) Mathematical formulation describing the connection between linear regression problems with quadratic regularization and quadratic integral-type loss (\textbf{top}), the generalized Hopf formula for an HJ PDE with quadratic time-dependent Hamiltonian and quadratic initial condition (\textbf{middle}), and an LQR problem with time-dependent running costs and dynamics (\textbf{bottom}). The content of this illustration is a special case of the connection in Figure~\ref{fig:connection_general} using a quadratic data fitting loss and quadratic regularization. We use this connection to develop our Riccati-based methodology (Section~\ref{sec:method}) and perform our numerical examples (Section~\ref{sec:examples}). The colors indicate the associated quantities between each problem. The solid-line arrows denote direct equivalences. The dotted arrows represent additional mathematical relations.}
    \label{fig:connection_Riccati_learning}
\end{figure}

The learning problem is formulated as follows. Given data $(s, \by(s))\in [0,t]\times \LPoutspace$ and boundary conditions $(s,\bz_s)\in \{0,t\}\times \LPoutspace$, the goal is to learn a linear prediction model $\Phi(s)\weightvec$ such that $\mathcal{A}\Phi(s)\weightvec \approx \by(s), \forall s\in[0,t]$ and $\mathcal{B}_s\Phi(s)\weightvec \approx \bz_s, s=0,t$, where $\Phi(s) = [\phi_1(s), ..., \phi_n(s)]\in\R^{m\times n}$ is the matrix whose columns are the basis functions $\phi_j:[0,t]\to\R^m$, $j=1, \dots, n$ evaluated at $s$, $\weightvec = [\weight_1, \dots, \weight_n]^T\in\Rn$ are unknown trainable coefficients, and $\mathcal{A}, \mathcal{B}_0, \mathcal{B}_t:\LPoutspace\to\LPoutspace$ are linear operators (e.g., identity operator, differential operators), where we follow the usual convention and denote by $\mathcal{A}\Phi(s)$ the matrix resulting from applying $\mathcal{A}$ to each column of $\Phi(s)$ (and similarly for $\mathcal{B}_0, \mathcal{B}_t$). The unknown coefficients $\weightvec$ are learned by minimizing the following loss function:
\begin{equation}\label{eq:loss_function}
    \mathcal{L}(\weightvec) = \int_0^t\frac{\lambda}{2}\|\mathcal{A}\Phi(s)\weightvec - \MLy(s)\|_2^2 ds + \frac{\lambda_0}{2}\|\mathcal{B}_0\Phi(0)\weightvec - \bz_0\|_2^2 + \frac{\lambda_t}{2}\|\mathcal{B}_t\Phi(t)\weightvec - \bz_t\|_2^2 + \frac{1}{2}\sum_{i=1}^n\MLreg_i (\weight_i - \MLcenter_i)^2,
\end{equation}
where $\lambda\geq0$ is a hyper-parameter for the data fitting term, $\lambda_0,\lambda_t\geq0$ are hyper-parameters for the boundary terms, $\MLreg_i>0, i=1,...,n$ are hyper-parameters for the regularization terms, and $\MLcenter_i \in \R$ is a prior on the unknown coefficients that biases $\weight_i$ to be close to $\MLcenter_i$. Note that the above loss function~\eqref{eq:loss_function} is strictly convex, and hence it has a unique global minimizer. 

Then, this learning problem has connections with a generalized Hopf formula and an associated optimal control problem. This connection is summarized in Figure~\ref{fig:connection_Riccati_learning}. Specifically, by completing the square, we see that computing the minimizer of the loss function~\eqref{eq:loss_function} is equivalent to computing the maximizer of the following generalized Hopf formula:
\begin{equation}\label{eq:genHopf_quad}
\begin{aligned}
    S(\HJx, \HJt) & = \sup_{\HJmom\in\Rn}\left\{\langle\HJx,\HJmom\rangle- \int_0^\HJt \frac{\lambda}{2}\|\mathcal{A}\Phi(s)\HJmom - \by(s)\|_2^2\,ds - \frac{1}{2}\|M^{1/2}\HJmom\|_2^2 + \langle\lambda_0(\mathcal{B}_0\Phi(0))^T\bz_0,\HJmom\rangle\right\},
\end{aligned}
\end{equation}
when $\HJx = \lambda_t(\mathcal{B}_t\Phi(t))^T\bz_t +\MLregmat\MLcentervec$, where $\MLregmat\in\R^{n\times n}$ is the diagonal matrix whose $i$-th entry is $\MLreg_i$ and $M = \lambda_0(\mathcal{B}_0\Phi(0))^T\mathcal{B}_0\Phi(0) + \lambda_t(\mathcal{B}_t\Phi(t))^T\mathcal{B}_t\Phi(t) + \MLregmat$. In other words, solving this learning problem~\eqref{eq:loss_function} is equivalent to solving the HJ PDE~\eqref{eq:HJPDE_timedependent} with time-dependent, quadratic Hamiltonian $\Hamiltonian(s,\HJmom) = \frac{\lambda}{2}\|\mathcal{A}\Phi(s)\HJmom - \by(s)\|_2^2$ and quadratic initial condition $\HJIC(\HJx) = \frac{1}{2}\HJx^T M^{-1}\HJx$ at the point $(\lambda_0(\mathcal{B}_0\Phi(0))^T\bz_0 + \lambda_t(\mathcal{B}_t\Phi(t))^T\bz_t +\MLregmat\MLcentervec,t)$. By extension, solving both of these problems is also equivalent to solving the optimal control problem~\eqref{eq:opt_ctrl} with running cost $L(s,\HJu) = \frac{1}{2}\HJu^T\HJu - \sqrt{\lambda}\by(s)^T\HJu$, terminal cost $\HJIC(\HJx) = \frac{1}{2}\HJx^TM^{-1}\HJx$, dynamics $f(s,\HJu) = \sqrt{\lambda}(\mathcal{A}\Phi(s))^T\HJu$, initial position $\HJx(0) = \lambda_0(\mathcal{B}_0\Phi(0))^T\bz_0 + \lambda_t(\mathcal{B}_t\Phi(t))^T\bz_t+ \MLregmat\MLcentervec$, and time horizon $\HJt$. Note that since this optimal control problem has quadratic running and terminal costs and linear dynamics, it is actually an LQR problem with time-dependent costs and dynamics. 

---------------------------------------------------------------------------------------------------------------------------

\update{TEMPORARY CALCULATIONS: to enforce boundary conditions}\begin{align*}
        \mathcal{L}(\weightvec) = \int_0^t\frac{1}{2}\|\Phi(s)\weightvec - \MLy(s)\|_2^2 ds + \frac{\lambda_0}{2}\|\Phi(0)\weightvec - \MLy(0)\|_2^2 + \frac{\lambda_t}{2}\|\Phi(t)\weightvec - \MLy(t)\|_2^2 +  \frac{1}{2}\|\MLregmat^{1/2}(\weightvec - \MLcentervec)\|_2^2 
\end{align*}
\begin{align*}
    &\frac{\lambda_0}{2}\|\Phi(0)\weightvec - \MLy(0)\|_2^2 + \frac{\lambda_t}{2}\|\Phi(t)\weightvec - \MLy(t)\|_2^2 +  \frac{1}{2}\|\MLregmat^{1/2}(\weightvec - \MLcentervec)\|_2^2 \\
    &= \frac{\lambda_0}{2}\left(\langle\weightvec, \Phi(0)^T\Phi(0)\weightvec \rangle - 2\langle\weightvec,\Phi(0)^T\MLy(0)\rangle + \|\MLy(0)\|^2\rangle\right) \\
    & + \frac{\lambda_t}{2}\left(\langle\weightvec, \Phi(t)^T\Phi(t)\weightvec \rangle - 2\langle\weightvec,\Phi(t)^T\MLy(t)\rangle + \|\MLy(t)\|^2\rangle\right) + \frac{1}{2}\left(\langle \weightvec, \MLregmat\weightvec\rangle - 2\langle\weightvec,\MLregmat\MLcentervec\rangle + \|\MLregmat^{1/2}\MLcentervec\|^2\right) \\
    & = \frac{1}{2}\left(\|(\lambda_0\Phi(0)^T\Phi(0) + \lambda_t\Phi(t)^T\Phi(t)) + \MLregmat)^{1/2}\weightvec\|^2 - 2\langle\weightvec, \lambda_0\Phi(0)^T\MLy(0) + \lambda_t\Phi(t)^T\MLy(t)+ \MLregmat\MLcentervec\rangle\right) + C \\
    & = \frac{1}{2}\|M^{1/2}(\weightvec - M^{-1}\bb)\|^2 + C, 
\end{align*}
where $M = \lambda_0\Phi(0)^T\Phi(0) + \lambda_t\Phi(t)^T\Phi(t)) + \MLregmat$ and $\bb = \lambda_0\Phi(0)^T\MLy(0) + \lambda_t\Phi(t)^T\MLy(t)+ \MLregmat\MLcentervec$.
So minimizing $\mathcal{L}(\weightvec)$ is equivalent to minimizing 
$$\int_0^t\frac{1}{2}\|\Phi(s)\weightvec - \MLy(s)\|_2^2 ds +  \frac{1}{2}\|M^{1/2}(\weightvec - M^{-1}\bb)\|_2^2$$
The corresponding HJ PDE then has Hamiltonian $\Hamiltonian(s,\HJmom) = \frac{1}{2}\|\Phi(s)\HJmom - \by(s)\|_2^2$ and initial condition $\HJIC(\HJx) = \frac{1}{2}\HJx^TM^{-1}\HJx$, and we evaluate the HJ PDE at $(\HJx,t) = (\bb, t)$. The generalized Hopf formula is 
$$S(\HJx, \HJt)= -\inf_{\HJmom\in\Rn}\left\{\int_0^\HJt \frac{1}{2}\|\Phi(s)\HJmom - \by(s)\|_2^2\,ds + \frac{1}{2}\|M^{1/2}\HJmom\|_2^2 - \langle\HJx,\HJmom\rangle\right\}.$$
The Riccati ODEs are then the same as~\eqref{eqt:RiccatiODEs} but with the initial conditions $\Sxx(0) = M^{-1}$ and $\Sx(0) = 0$.

---------------------------------------------------------------------------------------------------------------------------

%where $\MLreg_i>0, i=1,...,n$ are tunable hyper-parameters for the regularization terms and $\MLcenter_i \in \R$ is a prior on the unknown coefficients that biases $\weight_i$ to be close to $\MLcenter_i$. Note that the above loss function~\eqref{eq:loss_function} is strictly convex, and hence it has a unique global minimizer. 

%Then, this learning problem has connections with a generalized Hopf formula and an associated optimal control problem. This connection is summarized in Figure~\ref{fig:connection_Riccati_learning}. Specifically, solving this learning problem~\eqref{eq:loss_function} is related to solving the HJ PDE~\eqref{eq:HJPDE_timedependent} with time-dependent, quadratic Hamiltonian $\Hamiltonian(s,\HJmom) = \frac{1}{2}\|\Phi(s)\HJmom - \by(s)\|_2^2$ and quadratic initial condition $\HJIC(\HJx) = \frac{1}{2}\HJx^T\MLregmat^{-1}\HJx$, where $\MLregmat\in\R^{n\times n}$ is the diagonal matrix whose $i$-th entry is $\MLreg_i$. The viscosity solution to this HJ PDE is  given by the following generalized Hopf formula:
%\begin{equation}\label{eq:genHopf_quad}
%\begin{aligned}
 %   S(\HJx, \HJt) %& = \sup_{\HJmom\in\Rn}\left\{\langle\HJx,\HJmom\rangle - \int_0^\HJt \frac{1}{2}\|\Phi(s)\HJmom - \by(s)\|_2^2\,ds - \frac{1}{2}\|\MLregmat^{1/2}\HJmom\|_2^2\right\} \\
  %  & = -\inf_{\HJmom\in\Rn}\left\{\int_0^\HJt \frac{1}{2}\|\Phi(s)\HJmom - \by(s)\|_2^2\,ds + \frac{1}{2}\|\MLregmat^{1/2}\HJmom\|_2^2 - \langle\HJx,\HJmom\rangle\right\}.
%\end{aligned}
%\end{equation}
%From this representation formula~\eqref{eq:genHopf_quad}, we see that computing the minimizer of~\eqref{eq:loss_function} is equivalent to computing the minimizer of the right-hand side of~\eqref{eq:genHopf_quad} when $\HJx = \MLregmat\MLcentervec$; i.e., solving the regularized linear regression problem~\eqref{eq:loss_function} is equivalent to evaluating the corresponding HJ PDE at $(\HJx,t) = (\MLregmat\MLcentervec,t)$. By extension, solving both of these problems is also equivalent to solving the optimal control problem~\eqref{eq:opt_ctrl} with running cost $L(s,\HJu) = \frac{1}{2}\HJu^T\HJu - \by(s)^T\HJu$, terminal cost $\HJIC(\HJx) = \frac{1}{2}\HJx^T\MLregmat^{-1}\HJx$, dynamics $f(s,\HJu) = \Phi(s)^T\HJu$, initial position $\HJx(0) = \MLregmat\MLcentervec$, and time horizon $\HJt$. Note that since this optimal control problem has quadratic running and terminal costs and linear dynamics, it is actually an LQR problem with time-dependent costs and dynamics. 

It is well-known that LQR problems can be solved using the Riccati ODEs. By our connection, this gives us that the learning problem~\eqref{eq:loss_function} can also be solved using the Riccati ODEs. 
Namely, the minimizer $\weightvec^*$ of the learning problem~\eqref{eq:loss_function} is given by 
\begin{equation}
    \weightvec^* = \HJmom^* = \nabla_\HJx S(\MLregmat\MLcentervec,t) = \Sxx(t)\MLregmat\MLcentervec + \Sx(t),
\end{equation}
where $\HJmom^*$ is the optimizer in the generalized Hopf formula~\eqref{eq:genHopf_quad} when $\HJx = \MLregmat\MLcentervec$ and  
%the solution to the HJ PDE is given by $S(\HJx,\HJt) = \frac{1}{2}\HJx^T\Sxx(t)\HJx + \Sx(t)^T\HJx + \Sc(t)$, where 
$\Sxx:\R\to\R^{n\times n}$, which takes values in the space of positive definite matrices, and $\Sx:\R\to\Rn$ %, and $\Sc:\R\to\R$ 
satisfy the following Riccati ODEs:
\begin{equation}\label{eqt:RiccatiODEs}
    \begin{dcases}
    \dot{\Sxx}(s) =  -\Sxx(s)^T\MLbasismat(s)^T\MLbasismat(s)\Sxx(s) &s>0,\\
    \dot{\Sx}(s) = -\Sxx(s)^T\MLbasismat(s)^T(\MLbasismat(s)\Sx(s) - \MLy(s))&s>0%, \\
   % \dot{\Sc}(s) = -\frac{1}{2}\left\|\MLbasismat(s)\Sx(s)- \by(s)\right\|_2^2 & s > 0
    \end{dcases}
\end{equation}
with initial conditions $\Sxx(0) = \MLregmat^{-1}$ and $\Sx(0) = 0$.%, and $\Sc(0) = 0$.

==> BC-versions/theory.tex <==
In this section, we establish a new theoretical connection between regularized learning problems with integral-type losses, the generalized Hopf formula for HJ PDEs with time-dependent Hamiltonians, and optimal control problems. We begin by introducing the generalized Hopf formula and reviewing the well-established connections between HJ PDEs and optimal control. Then, we introduce the learning problems of interest and formulate our new theoretical connection.

\subsection{Generalized Hopf formula for HJ PDEs with time-dependent Hamiltonians}
Consider the following HJ PDE with time-dependent Hamiltonian:
\begin{equation}\label{eq:HJPDE_timedependent}
    \begin{dcases}
        \frac{\partial S(\HJx, \HJt)}{\partial \HJt} + \Hamiltonian(\HJt, \nabla_\HJx S(\HJx, \HJt)) = 0 & \HJx\in\Rn, \HJt > 0, \\
        S(\HJx, 0) = \HJIC(\HJx) & \HJx\in\Rn,
    \end{dcases}
\end{equation}
where $\Hamiltonian:(0,\infty)\times\Rn\to \R$ is the Hamiltonian and $J:\Rn\to\R$ is the initial condition. Assume that $\Hamiltonian, \HJIC$ are continuous, $\HJIC$ is convex, and $\Hamiltonian(\HJt,\HJmom)$ is convex in $\HJmom$. Then, using the same proof as that for \cite[Proposition 1]{lions1986hopf}, it can be shown that the viscosity solution to this HJ PDE~\eqref{eq:HJPDE_timedependent} can be represented by the following generalized Hopf formula:
\begin{equation}\label{eq:generalizedHopf}
    S(\HJx, \HJt) = \sup_{\HJmom\in\Rn}\left\{\langle\HJx,\HJmom\rangle - \int_0^\HJt \Hamiltonian(s,\HJmom)ds - \HJIC^*(\HJmom)\right\} = -\inf_{\HJmom\in\Rn}\left\{\int_0^\HJt \Hamiltonian(s,\HJmom)ds + \HJIC^*(\HJmom) - \langle\HJx,\HJmom\rangle\right\},
\end{equation}
where $f^*$ denotes the Fenchel-Legendre transform of the function $f$; i.e., $f^*(\HJmom) = \sup_{\HJx\in\Rn} \{\langle \HJx, \HJmom\rangle - f(\HJx)\}$. Note that if the integral in~\eqref{eq:generalizedHopf} is discretized in time, then we recover a multi-time Hopf formula (e.g., see \cite{rochet1985multitimeHJ, lions1986hopf, chen2023leveraging, darbon2019decomposition}), and hence,~\eqref{eq:HJPDE_timedependent} can also be considered as a multi-time HJ PDE with infinitely many times. 

It is well-known that the value function of the following optimal control problem also satisfies the HJ PDE~\eqref{eq:HJPDE_timedependent}:
\begin{equation}\label{eq:opt_ctrl}
    S(\HJx,\HJt) = \min_{\HJu(\cdot)}\left\{\int_0^\HJt L(s, \HJu(s))ds + \HJIC(\bx(\HJt)): \dot\bx(s) = f(s, \HJu(s)) \forall s\in(0,\HJt], \bx(0) = \HJx\right\},
\end{equation}
where $\HJx$ is the initial position, $\HJt$ is the time horizon, $\HJu(\cdot)$ is a control, $\bx(\cdot)$ is a trajectory, the running cost $L$ and the source term $f$ of the dynamics are related to the Hamiltonian $\Hamiltonian$ by $\Hamiltonian(s,\HJmom) = \sup_{\HJu\in\R^m} \{\langle -f(s,\HJu), \HJmom\rangle - L(s,\HJu)\}$, and $\HJIC$ is now regarded as the terminal cost.


\begin{proposition}\update{PC: this proposition may be commented out in the final paper...} 
    If $\Hamiltonian,\HJIC$ are continuous, $\HJIC$ is convex, and $\Hamiltonian(\HJt,\HJmom)$ is convex in $\HJmom$, then the generalized Hopf formula~\eqref{eq:generalizedHopf} is the viscosity solution to the time-dependent HJ PDE~\eqref{eq:HJPDE_timedependent}.
\end{proposition}

\begin{proof}
    We follow the proof for \cite[Proposition 1]{lions1986hopf}. To do so, we will show that~\eqref{eq:generalizedHopf} is both a viscosity subsolution and viscosity supersolution of~\eqref{eq:HJPDE_timedependent}, where we use the characterization of viscosity (sub-/super-) solutions using generalized gradients \cite[Proposition I.18]{crandall1983viscosity}. Namely, $S$ is viscosity subsolution (supersolution, resp.) of~\eqref{eq:HJPDE_timedependent} if and only if for all $(\HJx_0, t_0)\in\Rn\times[0,\infty)$ and for every $(\bp,q)$ in the superdifferential (subdifferential, resp.) of $S$ at $(\HJx_0, t_0)$, $q + H(t_0, \bp) \geq 0$ ($\leq 0$, resp.). $S$ is a viscosity solution if it is both a viscosity subsolution and viscosity supersolution. 
    
    First, we will show that~\eqref{eq:generalizedHopf} is a viscosity subsolution of~\eqref{eq:HJPDE_timedependent}. Note that the generalized Hopf formula~\eqref{eq:generalizedHopf} can equivalently be written as 
    \begin{equation}
        S(\HJx, \HJt) = \left(\HJIC^* + \int_0^\HJt \Hamiltonian(s,\cdot)ds\right)^*(\HJx).
    \end{equation}
    From this formulation, it is clear that~\eqref{eq:generalizedHopf} is a convex function satisfying~\eqref{eq:HJPDE_timedependent} at every point of differentiability. Since all convex functions are subdifferentiable, if $S$ is superdifferentiable at $(\HJx_0, t_0)$, then it is also differentiable at that point and hence, $q + H(t_0, \bp) = \frac{\partial S(\HJx_0,t_0)}{\partial t} + H(t_0,\nabla_\HJx S(\HJx_0,t_0)) = 0$ for all $(\bp,q)$ in the superdifferential of $S$ at $(\HJx_0, t_0)$. In other words, $S$ is a viscosity subsolution.

    Next, we will show that~\eqref{eq:generalizedHopf} is a viscosity supersolution of~\eqref{eq:HJPDE_timedependent}. Denote by $\Bar{S}_H(t_1,t_2)$, the operator $\Bar{S}_H(t_1,t_2)f = (f^* + \int_{t_1}^{t_2} H(\lambda, \cdot)d\lambda)^*$. Then, for all $s\in [0, t_0]$, we have that 
    \begin{equation} \label{eq:prop1_semigroup_identity}
        \begin{aligned}
            \left[\Bar{S}_H(t_0-s,t_0) S(\cdot, t_0-s)\right](\HJx_0) & = \left(S^*(\cdot, t_0-s) + \int_{t_0-s}^{t_0} H(\lambda, \cdot)d\lambda\right)^*(\HJx_0) \\
            & = \left( \left(\HJIC^* + \int_0^{\HJt_0-s} \Hamiltonian(\lambda,\cdot)d\lambda\right)^{**} + \int_{t_0-s}^{t_0} H(\lambda, \cdot)d\lambda\right)^*(\HJx_0) \\
            & = \left( \HJIC^* + \int_0^{\HJt_0-s} \Hamiltonian(\lambda,\cdot)d\lambda + \int_{t_0-s}^{t_0} H(\lambda, \cdot)d\lambda\right)^*(\HJx_0) \\
            & = \left( \HJIC^* + \int_0^{\HJt_0} \Hamiltonian(\lambda,\cdot)d\lambda\right)^*(\HJx_0) \\
            & = S(\HJx_0, t_0),
        \end{aligned}
    \end{equation}
    where the third equality follows from $f^{**} = f$ when $f$ is convex. Let $(\bp,q)$ be in the subdifferential of $S$ at $(\HJx_0,t_0)$. Then, by the definition of subdifferentials, we have that for all $(\HJx,t)\in\Rn\times[0,\infty)$,
    $$S(\HJx,t) \geq S(\HJx_0,t_0) + \langle \bp, \HJx-\HJx_0\rangle + q(t-t_0).$$
    In particular, taking $t = t_0 - s$ and applying $\Bar{S}_H(t_0-s,t_0)$ to both sides (note that $\Bar{S}_H(t_1,t_2)$ is order-preserving for all $t_1,t_2$ since the Fenchel-Legendre transform is order-reversing: $f\leq g \implies f^*\geq g^* \implies f^* + \int H(\lambda,\cdot)d\lambda \geq g^*  + \int H(\lambda,\cdot)d\lambda \implies  (f^* + \int H(\lambda,\cdot)d\lambda)^* \leq (g^*  + \int H(\lambda,\cdot)d\lambda)^*$) gives
    \begin{equation}\label{eq:prop1_inequality}
    \begin{aligned}
        S(\HJx_0, t_0) & = \left[\Bar{S}_H(t_0-s,t_0)S(\cdot,t_0-s)\right](\HJx_0) \\
        & \geq  \left[\Bar{S}_H(t_0-s,t_0)\phi\right](\HJx_0) = \sup_{\bz\in\Rn}\left\{ \langle \bz,\HJx_0\rangle - \int_{t_0-s}^{t_0} H(\lambda,\bz)d\lambda - \phi^*(\bz)\right\},
    \end{aligned}
    \end{equation}
    where the first equality follows from~\eqref{eq:prop1_semigroup_identity}, we define $\phi(\HJx) = S(\HJx_0,t_0) + \langle \bp, \HJx-\HJx_0\rangle -sq$, and the second equality follows from the definitions of $\Bar{S}_H(t_0-s,t_0)$ and the Fenchel-Legendre transform.
    Now note that 
    \begin{equation}
    \begin{aligned}
    \phi^*(\bz) & = \sup_{\HJx\in\Rn} \{\langle \HJx,\bz\rangle - S(\HJx_0,t_0) - \langle \bp, \HJx-\HJx_0\rangle + sq\} \\
        & = \begin{dcases}
            sq - S(\HJx_0,t_0) + \langle \bp, \HJx_0\rangle & \bz = \bp \\
            +\infty & \bz\neq \bp.
        \end{dcases}
    \end{aligned}
    \end{equation}
    Combining this fact with~\eqref{eq:prop1_inequality} gives us that
    \begin{equation}
        S(\HJx_0,t_0) \geq \langle \bp,\HJx_0\rangle - \int_{t_0-s}^{t_0} H(\lambda,\bp)d\lambda - \phi^*(\bp) = S(\HJx_0,t_0) - sq - \int_{t_0-s}^{t_0} H(\lambda,\bp)d\lambda.
    \end{equation}
    Rearranging terms gives us that
    $$q + \frac{1}{s}\int_{t_0-s}^{t_0} H(\lambda,\bp)d\lambda \geq 0.$$
    Letting $s\to 0$, we have that $q + H(t_0,\bp) \geq 0$, or in other words, $S$ is a viscosity supersolution. 
\end{proof}

\subsection{Connection to learning problems}
\begin{figure}[htbp]

    \centering   
    \begin{adjustbox}{width=\textwidth}
\begin{tikzpicture}[node distance=2cm]
    \node (min) [nobox, yshift=-0.2cm] {$\min$};
    \node (minarg) [boxsmall, right of=min, xshift=-1.3cm, yshift=-0.42cm, draw=cyan!60, fill=cyan!5] {$\text{}_{\weightvec\in\weightspace}$};
    \node (sum) [nobox, right of=min, xshift=-0.32cm] {$\mathlarger{\int}_0^t$};
    \node (loss) [box, right of=sum, xshift=0.1cm, draw=green!60, fill=green!5] {$\lambda\lossfunc(\mathcal{A}F(s;\weightvec), \by(s))$};
    \node(ds) [nobox, right of=loss, xshift=-0.0cm] {$ds$};
    \node (plus) [nobox, right of=loss, xshift=0.5cm] {$+$};
    \node (regLeft) [nobox, right of=loss, xshift=4.5cm, draw=blue!60, fill=blue!5] {$\lambda_0\lossfunc_0(\mathcal{B}_0F(0;\weightvec), \bz_0)+ \lambda_t\lossfunc_t(\mathcal{B}_tF(t;\weightvec), \bz_t)$};
    \node (regularization) [nobox, right of=regLeft, xshift=1.9cm] {$+$};
    \node (regRight) [nobox, right of=regularization, xshift=-1.2cm, draw=blue!60, fill=blue!5] {$\regfunc(\weightvec)$};
    
    \node (sup) [nobox, below of=min, xshift=-0cm] {$\min$};
    \node (suparg) [boxsmall, right of=sup, xshift=-1.3cm, yshift=-0.44cm, draw=cyan!60, fill=cyan!5] {$\text{}_{\HJmom\in\HJstatespace}$};
    \node (sum2) [nobox, below of=sum,xshift=0.95cm]{$\mathlarger{\int}_0^t$};
    \node (equal) [nobox, left of=sup, xshift=1.4cm] {$=$};
    \node (S) [box, left of=equal, xshift=0.45cm, draw=red!60, fill=red!5] {$S(\HJx, \HJt)$};
    \node (minus) [nobox, left of=S, xshift=1.1cm] {$-$};
    \node (Hamiltonian) [box, below of=loss, draw=green!60, fill=green!5] {$\Hamiltonian(s,\HJmom)$};
    \node(HJds) [nobox, below of=ds, xshift=-0.94cm] {$ds$};
    \node (plus2) [nobox, right of=Hamiltonian, xshift=1.5cm] {$+$};
    \node (IC) [box, below of=regLeft, xshift=0cm, draw=blue!60, fill=blue!5] {$\HJIC^*(\HJmom)$};
    \node (linear) [box, below of=regRight, draw=blue!60, fill=blue!5] {$-\langle \HJx, \HJmom\rangle$};

    \node (OCmin) [nobox, below of=sup, xshift=0cm] {$\min$};
    \node (OCminarg) [boxsmall, below of=suparg, yshift=-0.01cm, draw=cyan!60, fill=cyan!5] {$\text{}_{\HJu(\cdot)}$};
    \node (OCS) [box, below of=S, xshift=0cm, draw=red!60, fill=red!5] {$S(\HJx, \HJt)$};
    \node (leftbracket) [nobox, right of=OCmin, xshift=0.02cm] {$\Bigg\{$};
    \node (OCequal) [nobox, below of=equal] {$=$};
    \node (OCint) [nobox, below of=sum2, xshift=-0.18cm] {$\mathlarger{\int}_0^t$};
    \node (OCHamiltonian) [box, below of=Hamiltonian, draw=green!60, fill=green!5] {$L(s,\HJu(s)) $};
    \node (OCds) [nobox, right of=OCHamiltonian, xshift=-0.75cm] {$ds$};
    \node (OCplus) [nobox, right of=OCds, xshift=-1.0 cm] {$+$};
    \node (OCIC) [box, below of=IC, draw=blue!60, fill=blue!5, xshift=-2.6cm] {$\HJIC\left(\bx\left(\HJt\right)\right)$};
    \node (colon) [nobox, right of=OCIC, xshift=-1.1cm] {:};
    \node(OCdynamics) [box, right of=OCIC, xshift=1.6cm, draw=green!60, fill=green!5] {$\dot\bx(s) = f(s,\HJu(s)), \forall s \in \left(0, \HJt\right]$};
    \node(comma) [nobox, right of=OCdynamics, xshift=0.55cm, yshift=-0.11cm] {,};
    \node (terminalposition) [box, right of=OCdynamics, xshift=1.7cm, draw=blue!60, fill=blue!5] {$\bx\left(0\right) = \HJx$};
    \node (rightbracket) [nobox, right of=terminalposition, xshift=-0.92cm] {$\Bigg\}$};

    \node (LPequal) [nobox, above of=equal] {$=$};
    \node (minloss) [box, above of=S, draw=red!60, fill=red!5] {$\min_{\weightvec\in\weightspace}\mathcal{L}(\weightvec)$};
    
    \draw [doublearrow] (loss) -- (Hamiltonian);
    \draw [dottedarrow] (regLeft) -- (IC);
    \draw [dottedarrow] (regLeft) -- (linear);
    \draw [dottedarrow] (regRight) -- (IC);
    \draw [dottedarrow] (regRight) -- (linear);
    \draw [doublearrow] (minarg) -- (suparg);
    \draw [doublearrow] (S) -- (OCS);
    \draw [dottedarrow] (IC) -- (OCIC);
    \draw [dottedarrow] (Hamiltonian) -- (OCHamiltonian);
    \draw [dottedarrow] (Hamiltonian) -- (OCdynamics);
    \draw [dottedarrow] (linear) -- (terminalposition);
    \draw[dottedarrow](minloss) -- (S);
    \draw[dottedarrow] (suparg) -- (OCminarg);
\end{tikzpicture}
\end{adjustbox}

    \caption{(See Section~\ref{sec:theory}) Mathematical formulation describing the connection between a regularized learning problem with integral-type loss (\textbf{top}), the generalized Hopf formula for HJ PDEs with time-dependent Hamiltonians (\textbf{middle}), and the corresponding optimal control problem (\textbf{bottom}). The content of this illustration matches that of Figure~\ref{fig:intro_connection_in_words} by replacing each term in Figure~\ref{fig:intro_connection_in_words} with its corresponding mathematical expression. The colors indicate the associated quantities between each problem. The solid-line arrows denote direct equivalences. The dotted arrows represent additional mathematical relations.}
    \label{fig:connection_general}
\end{figure}

In this section, we connect the Hopf formula~\eqref{eq:generalizedHopf} with regularized learning problems with integral-type losses. Consider a learning problem with data $(s,\by(s)) \in [0,t]\times \LPoutspace$ and boundary data $(s,\bz_s) \in \{0,T\}\times \LPoutspace$, where $t\leq T$. The goal of the learning problem is to learn a function $F(s;\weightvec)$ with input $s\in[0,t]$ and unknown parameter $\weightvec\in\weightspace$. We learn $F$ as follows. First, we apply an operator $\mathcal{A}$ to the function $F$, such that $\mathcal{A}F(s;\weightvec) \approx \by(s), \forall s\in[0,t]$. For example, $\mathcal{A}$ could be the identity operator (as in regression problems; e.g., see \cite{weisberg2005applied}) or a differential operator (as in PINNs; e.g., see \cite{raissi2019physics}). The discrepancy between the learned model $\mathcal{A}F(s;\weightvec)$ and the measurements $\by(s)$ is measured using a integral-type data fitting loss $\int_0^t\lossfunc(\mathcal{A}F(s;\weightvec), \by(s))ds$, where we assume that the function $\weightvec \mapsto \lossfunc(\mathcal{A}F(s;\weightvec), \by(s))$ is convex. For example, setting $\lossfunc(\ba, \bb) = \|\ba-\bb\|_1 = \sum_{i=1}^m |a_i-b_i|$ or $\lossfunc(\ba, \bb) = \|\ba-\bb\|^2_2 = \sum_{i=1}^m (a_i-b_i)^2$ yields an $L^1$ or $L^2$-squared loss, respectively. To enforce the boundary conditions, we apply the operators $\mathcal{B}_0, \mathcal{B}_t$ to $F$ at the boundary points $s=0,T$, respectively, and measure the discrepancy between $\mathcal{B}_sF(s;\weightvec)$ and $\bz_s$ for $s=0,t$ using $\lossfunc_0$ and $\lossfunc_t$, respectively, where $\weightvec \mapsto \lossfunc_s(\mathcal{B}_sF(s;\weightvec), \bz_s)$ is assumed to be convex for both $s=0,t$. The unknown parameters $\weightvec$ are then learned by solving the following optimization problem:
\begin{equation}\label{eqt:general_learning}
\min_{\weightvec\in \weightspace} \lambda\int_0^t \lossfunc(\mathcal{A}F(s;\weightvec), \by(s))ds + \lambda_0\lossfunc_0(\mathcal{B}_0F(0;\weightvec), \bz_0)+ \lambda_t\lossfunc_t(\mathcal{B}_tF(t;\weightvec), \bz_t)+\regfunc(\weightvec), 
\end{equation}
% \begin{equation}\label{eqt:general_learning}
% \min_{\weightvec\in \weightspace} \lambda\int_0^t \lossfunc(\mathcal{A}F(s;\weightvec), \by(s))ds + \lambda_0\|A\theta - b\|^2, % say it could be a combination of BCs and regularization
% \end{equation}
where $\lambda, \lambda_0, \lambda_t\geq 0$ are weights for each of the loss terms and $R$ is a regularization term. Note that if we do not have access to the boundary data, then the corresponding weight can be set to 0.

Then, the connection between the learning problem~\eqref{eqt:general_learning}, the generalized Hopf formula~\eqref{eq:generalizedHopf}, and the optimal control problem~\eqref{eq:opt_ctrl} is summarized in Figure~\ref{fig:connection_general}. Specifically, the learning problem~\eqref{eqt:general_learning} is related to the generalized Hopf formula~\eqref{eq:generalizedHopf} by setting $\weightvec = \HJmom$, $\Hamiltonian(s,\HJmom) = \lambda\lossfunc(\mathcal{A}F(s;\HJmom), \by(s))$, and $\lambda_0\lossfunc_0(\mathcal{B}_0F(0;\HJmom), \bz_0)+ \lambda_t\lossfunc_t(\mathcal{B}_tF(t;\HJmom), \bz_t)+\regfunc(\HJmom) = \HJIC^*(\HJmom) - \langle \HJx,\HJmom\rangle + c(\HJx)$, where $c(\HJx)$ is a constant (possibly 0) that is independent of $\HJmom$ but may depend on $\HJx$. In other words, the spatial variable $\HJx$ in the HJ PDE becomes a hyper-parameter in the learning problem, and we can treat it as a constant when optimizing the learning problem~\eqref{eqt:general_learning} with respect to $\weightvec = \HJmom$. Hence, when we solve these learning problems, we also evaluate the solution to the HJ PDE~\eqref{eq:HJPDE_timedependent} at the point $(\HJx,\HJt)$, or equivalently, we solve the corresponding optimal control problem~\eqref{eq:opt_ctrl} with initial position $\HJx$ and time horizon $\HJt$. Conversely, when we solve the HJ PDE~\eqref{eq:HJPDE_timedependent}, the spatial gradient $\nabla_\HJx S(\HJx, \HJt)$ of the solution gives the minimizer $\weightvec^*$ of the learning problem~\eqref{eqt:general_learning}.

==> CHANGES <==
v1.30 (2022-02-09):

  * jmlrutils.sty:

    - fixed counter name in lemma definition when cleveref option on

v1.29 (2022-01-29):

  * jmlr.cls:

    - added cleveref option

    - fixed draft option

    - bug fix #168: Float-only last pages not counted for page numbering
       https://www.dickimaw-books.com/bugtracker.php?key=168

  * jmlrutils.sty:

    - added cleveref option

    - added \jmlralgorule

    - added \jmlrminsubcaptionwidth

  * jmlrbook.cls:

    - obsoleted (https://www.dickimaw-books.com/faq.php?itemlabel=latex20201009)
      Production editors will need to set the first page number
      of each article manually.

v1.28 (2020-09-21):

  * jmlr.cls:

   Bug fixes: 

    - fixed twoside option (which should be the default)

    - \thanks now uses mpfootnote instead of footnote counter
      with matching \footnotemark and \footnotetext optional
      arguments.

v1.27 (2020-03-26):

  * jmlrutils.sty:

    Bug fix: subfigure and subtable references were producing
    extraneous text (added check for LaTeX kernel version)

v1.26 (2020-01-31):

  * jmlr.cls:

    - removed \vbox from \@jmlrmaketitle to allow for extremely long
      author/affiliation list. Added \ignorespaces before \@author
      to allow for spacing the contents in the code for clarity
      at the start of a long author list.

v1.25 (2020-01-17):

  * jmlr.cls: 

    - Added check for graphics.sty 2019/07/01 (which now detokenizes
      filename)

  * jmlrutils.sty:

    - Added \proofname

v1.24 (2017-08-01):

  * moved non-class related code into new package jmlrutils.sty

  * fixed bug in \includeteximage

v1.23 (2017-03-09):

  * added pmlr class option

v1.22 (2015-04-11):

  * added oneside and twoside class options

v1.21 (2015-02-24):

  * jmlr.cls

    - added check for jmlr2e and pseudocode

    - fixed bug in \thanks to fix footnote marker issue if there's
      more than one \thanks

  * jmlrbook.cls

    - added \nopagebreak after \@editorialteam

v1.20 (2014-10-15):

  * jmlrbook.cls

    - added \jmlrprefaceheader, \jmlrlocation

v1.19 (2014-09-29):

  * jmlrbook.cls

    - changed \chapter* to \chapter in preface environment

v1.18 (2013-10-17):

  * jmlrbook.cls

    - patched to work with auxhook

    - added draft and final options

    - add \booklinebreak

  * jmlr.cls

    - Added calc and etoolbox as required packages

    - Added draft and final options and removed \ds@draft

    - Added starred version of \newtheorem

    - Added \theorembodyfont, \theoremheaderfont, \theorempostheader
      and \theoremsep

v1.17 (2012-05-30):

  * jmlr.cls

    - added \titletag

    - added warnings if obsolete font commands (such as \bf) used

  * jmlrbook.cls

    - added 'articlet' page style

    - \importarticle sets title page style to articlet

    - \importpaper disables \jmlryear, \jmlrworkshop, \jmlrvolume
      and \jmlrissue

    - html title page uses jmlrvolume instead of volume

    - added optional argument to \logo

v1.16 (2012-05-15):

  * jmlr.cls

    - added \@post@hyperref hook

  * jmlrbook.cls

    - added code to deal with \c@lenddoca clash

v1.15 (2012-05-12):

  * jmlrbook.cls

    - added 'algocf' and 'definition' counters to reset list in
      \zeroextracounters

    - added \theHalgocf

    - removed dependence on \ps@headings in \ps@jmlrbook

    - added \markleft

v1.14 (2012-04-24):

  * jmlrbook.cls

    - modified \jmlrwritepdfinfo to write book author and title
      information to aux file
    - fixed bug in fetching time zone information

v1.13 (2012-02-25):

  * jmlrbook.cls

    - added pdfxa option
    - added \jmlrwritepdfinfo
    - changed preface environment to use \chapter* instead of \chapter

  * jmlr.cls

    - added \@pre@hyperref hook

v1.12 (2012-01-05):

  * jmlr.cls

    - removed prehyperref package option.

    - renamed \jmlr@prehyperref to \jmlrprehyperref

    - added tabularx to list of problem packages.

    - provided default value of \@shortitle

    - added \titlebreak

    - added optional argument to \Name
      (\jmlrauthors now redefines \@jmlr@authors instead of
      \@jmlrauthors)

    - added chapter number to \theHsection to ensure unique
      hyperlinks in book

  * jmlrbook.cls

    - Moved loading setspace and fink before jmlr.cls loaded

    - changed \thechapter to \theHchapter in definition of
      \theHalgorithm etc

    - added \theHfootnote, \theHtable, \theHfigure

    - in \importpubpaper etc, changed \@shortitle to \@title in toc

  * makejmlrbook v0.31

    - footnotes in abstract files changed to in-line parentheses.

    - --batchtex option now also passes "-interaction=batchmode" to
      htlatex

    - added debugging option --noexecute

v1.11 (2011-03-24):

  * jmlr.cls

    - fixed typo: WC\&P -> W\&CP

    - added \jmlrabbrnamelist (used by makejmlrbook)

  * jmlrbook.cls

    - now requires fink package

    - added preface environment and \prefacename

    - added algorithm2e old commands (in case some authors are using
      an older version).

  * makejmlrbook (v0.3):

    - added changes made by Olivier Chapelle to add JMLR menu on the
      left side of the page and use description environment for each
      paper of the TOC.

    - added --extractpreface option

    - set hyperref draft mode for abstract only html pages.

    - abstract html source files now input original aux files to allow
      for citations.

v1.10 (2011-01-05):

  jmlr.cls

  * now loads xkeyval

  * now loads hyperref (instead of jmlrbook loading it)

  * added class option prehyperref={stuff to do before hyperref loaded}

  * added class option tablecaption=<position> (where <position> can
    either be top or bottom).

  * fixed 10pt, 11pt and 12pt class options, which weren't having
    any effect.

  * modified \thanks to ensure hyperlink works correctly.

  * added \mdseries to definition of \addr.

  * added \startpage (used by jmlrmakebook).

  * modified \artpart and \bookpart to correct bookmark level number

  jmlrbook.cls

  * code loading hyperref moved to jmlr.cls

  * added 10pt, 11pt and 12pt class options.

  * Removed redundant redefinition of \@bookpart

  makejmlrbook (v0.2):

  * Uses \startpage to set initial page number for stand-alone 
    articles.

  * Makes subdirectories in html directory for each article.

  * copies any image files generated by tex4ht into html directory.

  * added time stamp at the end of each of the generated html file.

v1.09 (2010-12-01):

  jmlr.cls

  * now loads article.cls instead of scrartcl.cls

  * Fixed sub-captions so that they don't exceed the width of the
    sub-figure/table to which they refer.

  * added \nametag, \reprint, \algocfconts, \theHsubfigure,
    \booktocpreamble, \@partapp.

  * Made \objectref robust

  jmlrbook.cls

  * Reset start and end document hook to avoid problems caused by
    defining duplicate commands.

  * Moved redefinition of \jmlrpremaketitlehook outside of import
    macros.

  * Moved \refstepcounter from \jmlrmaketitlehook to
    \jmlrpremaketitlehook

  * Added \jmlrimporthook

  * Added \label to \jmlrmaketitlehook

v1.08 (2010-07-27):

  * Fixed \thanks so that the footnote symbol is raised and isn't
    followed by a full stop.

v1.07 (2010-06-30):

  * Added check for two column

v1.06 (2010-06-17):

  jmlr.cls

  * Added tablecaptiontop and tablecaptionbottom class options

v1.05:

  jmlrbook.cls

  * Added \productioneditors

v1.04:

  * Added Perl script makejmlrbook

  jmlrbook.cls

  * Added patch to fix references in print mode

  * Added code to work with makejmlrbook

  jmlr.cls

  * Added code to work with makejmlrbook

v1.03:
  jmlrbook.cls

  * Added patch to combnat

  jmlr.cls

  * Added \editors, \editorname and \editorsname

v1.02:
  jmlrbook.cls:

  * Added \issue

  jmlr.cls

  * Added \jmlrissue

v1.01 :

  jmlrbook.cls: 

  * added \importpaper

  * added \titlebody, \SetTitleElement and \IfTitleElement to 
    make it easier to customise the front page of the book.

  jmlr.cls:

  * fixed the last page anchor.

v1.0 : Initial release


==> methodology_figure.tex <==
\begin{figure}[htbp]

    \centering   
    \begin{adjustbox}{width=\textwidth}
\begin{tikzpicture}[node distance=2cm]
    \node (min) [nobox, yshift=-0.2cm] {$\min$};
    \node (minarg) [boxsmall, right of=min, xshift=-1.3cm, yshift=-0.42cm, draw=cyan!60, fill=cyan!5] {$\text{}_{\weightvec\in\weightspace}$};
    \node (sum) [nobox, right of=min, xshift=0.4cm] {$\mathlarger{\int}_0^t$};
    \node (loss) [box, right of=sum, xshift=0.1cm, draw=green!60, fill=green!5] {$\frac{\lambda}{2}\|\mathcal{A}\Phi(s)\weightvec - \MLy(s)\|_2^2$};
    \node(ds) [nobox, right of=loss, xshift=0.02cm] {$ds$};
    \node (plus) [nobox, right of=loss, xshift=3.1cm] {$+$};
    \node (regLeft) [nobox, right of=loss, xshift=3cm] {};
    \node (regularization) [box, right of=regLeft, xshift=2.3cm, draw=blue!60, fill=blue!5] {$\frac{1}{2}\|\regmat\weightvec - \regcenter\|_2^2$};
    \node (regRight) [nobox, right of=regularization, xshift=2.35cm] {};
    
     \node (sup) [nobox, below of=min, xshift=-0cm] {$\min$};
    \node (suparg) [boxsmall, right of=sup, xshift=-1.3cm, yshift=-0.44cm, draw=cyan!60, fill=cyan!5] {$\text{}_{\HJmom\in\HJstatespace}$};
    \node (sum2) [nobox, below of=sum,xshift=0cm]{$\mathlarger{\int}_0^t$};
    \node (equal) [nobox, left of=sup, xshift=1.4cm] {$=$};
    \node (S) [box, left of=equal, xshift=0.45cm, draw=red!60, fill=red!5] {$S(0, \HJt)$};
    \node (minus) [nobox, left of=S, xshift=1.1cm] {$-$};
    \node (Hamiltonian) [box, below of=loss, draw=green!60, fill=green!5] {$\frac{\lambda}{2}\|\mathcal{A}\Phi(s)\HJmom - \by(s)\|_2^2$};
    \node(HJds) [nobox, below of=ds, xshift=0cm] {$ds$};
    \node (plus2) [nobox, right of=Hamiltonian, xshift=0.75cm] {$+$};
    \node (IC) [box, below of=regLeft, draw=blue!60, fill=blue!5] {$\frac{1}{2}\|\regmat\HJmom\|_2^2 - \langle\regmat\HJmom, \regcenter\rangle$};
    \node (linear) [box, below of=regRight, draw=blue!60, fill=blue!5] {$-\langle 0, \HJmom\rangle$};

    \node (OCmin) [nobox, below of=sup, xshift=0cm] {$\min$};
    \node (OCminarg) [boxsmall, below of=suparg, yshift=-0.0cm, draw=cyan!60, fill=cyan!5] {$\text{}_{\HJu(\cdot)}$};
    \node (OCS) [box, below of=S, xshift=0cm, draw=red!60, fill=red!5] {$S(0, \HJt)$};
    \node (leftbracket) [nobox, right of=OCmin, xshift=-0.65cm] {$\Bigg\{$};
    \node (OCequal) [nobox, below of=equal] {$=$};
    \node (OCint) [nobox, below of=sum2, xshift=-0.65cm] {$\mathlarger{\int}_0^t$};
    \node (OCHamiltonian) [box, below of=Hamiltonian, draw=green!60, fill=green!5] {$\frac{1}{2}\HJu(s)^T\HJu(s) - \sqrt{\lambda}\by(s)^T\HJu(s)$};
    \node (OCds) [nobox, right of=OCHamiltonian, xshift=0.68cm] {$ds$};
    \node (OCplus) [nobox, right of=OCds, xshift=-1.55cm] {$+$};
    \node (OCIC) [box, below of=IC, draw=blue!60, fill=blue!5] {$\frac{1}{2}\|(\regmat^{-1})^T\HJx + \regcenter\|_2^2$};
    \node (colon) [nobox, right of=OCIC, xshift=-0.35cm] {:};
    \node(OCdynamics) [box, right of=OCIC, xshift=2.7cm, draw=green!60, fill=green!5] {$\dot\bx(s) = \sqrt{\lambda}(\mathcal{A}\Phi(s))^T\HJu, \forall s \in \left(0, \HJt\right]$};
    \node(comma) [nobox, right of=OCdynamics, xshift=0.9cm, yshift=-0.11cm] {,};
    \node (terminalposition) [box, below of=linear, draw=blue!60, fill=blue!5] {$\bx\left(0\right) = 0$};
    \node (rightbracket) [nobox, right of=terminalposition, xshift=-0.95cm] {$\Bigg\}$};

    \node (LPequal) [nobox, above of=equal] {$=$};
    \node (minloss) [box, above of=S, draw=red!60, fill=red!5] {$\min_{\weightvec\in\weightspace}\mathcal{L}(\weightvec)$};
    
    \draw [doublearrow] (loss) -- (Hamiltonian);
    \draw [dottedarrow] (regularization) -- (IC);
    \draw [dottedarrow] (regularization) -- (linear);
    \draw [doublearrow] (minarg) -- (suparg);
    \draw [doublearrow] (S) -- (OCS);
    \draw [dottedarrow] (IC) -- (OCIC);
    \draw [dottedarrow] (Hamiltonian) -- (OCHamiltonian);
    \draw [dottedarrow] (Hamiltonian) -- (OCdynamics);
    \draw [dottedarrow] (linear) -- (terminalposition);
    \draw[dottedarrow](minloss) -- (S);
    \draw[dottedarrow] (suparg) -- (OCminarg);
\end{tikzpicture}
\end{adjustbox}

    \caption{(See Section~\ref{sec:method}) Mathematical formulation describing the connection between linear regression problems with quadratic regularization and quadratic integral-type loss (\textbf{top}), the generalized Hopf formula for an HJ PDE with quadratic time-dependent Hamiltonian and quadratic initial condition (\textbf{middle}), and an LQR problem with time-dependent running costs and dynamics (\textbf{bottom}). The content of this illustration is a special case of the connection in Figure~\ref{fig:connection_general} using a quadratic data fitting loss and quadratic regularization. We use this connection to develop our Riccati-based methodology (Section~\ref{sec:method}) and perform our numerical examples (Section~\ref{sec:examples}). The colors indicate the associated quantities between each problem. The solid-line arrows denote direct equivalences. The dotted arrows represent additional mathematical relations.}
    \label{fig:connection_Riccati_learning}
\end{figure}
